Arrhenius activation energy and transitivity in fission-track annealing equations

Fission-track annealing models aim to extrapolate laboratory annealing kinetics to the geological timescale for application to geological studies. Model trends empirically capture the mechanisms of track length reduction. To facilitate the interpretation of the fission-track annealing trends, a formalism, based on quantities already in use for the study of physicochemical processes, is developed and allows for the calculation of rate constants, Arrhenius activation energies, and transitivity functions for the fission-track annealing models. These quantities are then obtained for the parallel Arrhenius, parallel curvilinear, fanning Arrhenius, and fanning curvilinear models, fitted with Durango apatite data. Parallel models showed to be consistent with a single activation energy mechanism and a reaction order model of order ~ -4. However, the fanning curvilinear model is the one that results in better fits laboratory data and predictions in better agreement with geological evidence. Fanning models seem to describe a more complex picture, with concurrent recombination mechanisms presenting activation energies varying with time and temperature, and the reaction order model seems not to be the most appropriate. It is apparent from the transitivity analysis that the dominant mechanisms described by the fanning models are classical (not quantum) energy barrier transitions.

==> TableAnnealingData.tex <==
\begin{table*}[]
\caption{\label{tab:annealingdata}Adjustment coefficients to experimental data by annealing model.}
\setlength\tabcolsep{0pt} % let LaTeX compute intercolumn whitespace

\smallskip 
\begin{tabular*}{1.5\columnwidth}{@{\extracolsep{\fill}}cccccc}
\toprule
annealing model & $c_0$      & $c_1$     & $c_2$      & $c_3$     & $\chi_\nu^2$ \\
\midrule
 PA              & 5.631017  & 0.186520 & -10.455390 & -         & 2.65   \\
 PC             & -4.910332 & 0.194445  & -9.610091  & -         & 2.12   \\
 FA              & -8.51756 & 0.12659 & -20.99225 & 0.29845 & 1.66    \\
 FC             & -12.80664  & 0.23109   & -41.37987  & -1.20490  & 1.77  \\
\bottomrule
\end{tabular*}
\end{table*}
